Context-Augmented Software Development Projects: Literature Review and Preliminary Framework

Software development is a complex activity which depends on diverse technologies and people's expertise. The approaches to developing software highly depend on these different characteristics, which are the context developers are subject to. This context contains massive knowledge, and not capturing it means knowledge is continuously lost. Although extensively researched, context in software development is still not explicit, nor proposed into a broader view of the context needed by software developers and tools. Therefore, developers' productivity is affected, as the ability to reuse this rich context is hampered. This paper proposes a literature review on context for software development, through nine research questions. The purpose of this study is making the discovered context explicit into an integrated view and proposing a platform to aid software development using context information. We believe supporting contextual knowledge through its representation and mining for recommendation and real-time provision can significantly improve big data software project development.

==> ContextAugmented SDP (8)/authors.tex <==
\author{\IEEEauthorblockN{Glaucia Melo, Paulo Alencar, Don Cowan} 
\IEEEauthorblockA{\textit{David R. Cheriton School of Computer Science} \\
\textit{University of Waterloo}\\
Waterloo, Canada \\
\{gmelo,palencar, dcowan\}@uwaterloo.ca}
%\and
%\IEEEauthorblockN{Toacy Oliveira} 
%%\IEEEauthorblockA{
%\textit{PESC/COPPE} \\
%\textit{Universidade Federal}\\
%\textit{do Rio de Janeiro}\\
%Rio de Janeiro, Brazil \\
%toacy@cos.ufrj.br}
%\and
%\IEEEauthorblockN{Paulo Alencar} 
%\IEEEauthorblockA{
%\textit{David R. Cheriton} \\
%\textit{School of Computer Science} \\
%\textit{University of Waterloo}\\
%Waterloo, Canada \\
%palencar@uwaterloo.ca}
%\and
%\IEEEauthorblockN{Don Cowan}
%\IEEEauthorblockA{
%\textit{David R. Cheriton} \\
%\textit{School of Computer Science} \\
%\textit{University of Waterloo}\\
%Waterloo, Canada \\
%dcowan@uwaterloo.ca}
% \and
% \IEEEauthorblockN{4\textsuperscript{th} Given Name Surname}
% \IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
% \textit{name of organization (of Aff.)}\\
% City, Country \\
% email address}
% \and
% \IEEEauthorblockN{5\textsuperscript{th} Given Name Surname}
% \IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
% \textit{name of organization (of Aff.)}\\
% City, Country \\
% email address}
% \and
% \IEEEauthorblockN{6\textsuperscript{th} Given Name Surname}
% \IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
% \textit{name of organization (of Aff.)}\\
% City, Country \\
% email address}
}
